Josephson junction with magnetic-field tunable current-phase relation

We consider a 0-$\pi$ Josephson junction consisting of asymmetric 0 and $\pi$ regions of different lengths $L_0$ and $L_\pi$ having different critical current densities $j_{c,0}$ and $j_{c,\pi}$. If both segments are rather short, the whole junction can be described by an \emph{effective} current-phase relation for the spatially averaged phase $\psi$, which includes the usual term $\propto\sin(\psi)$, a \emph{negative} second harmonic term $\propto\sin(2\psi)$ as well as the unusual term $\propto H \cos\psi$ tunable by magnetic field $H$. Thus one obtains an electronically tunable current-phase relation. At H=0 this corresponds to the $\varphi$ Josephson junction.

==> MyMc.tex <==
%%% This is 'MyMc.tex' v3.00
%%% LaTeX macros for frequently used abbreviations
%%% 13.12.2011 by Edward Goldobin <gold@uni-tuebingen.de>

\RequirePackage{xspace}

%stupid macros like \ie, \eg, \etc
\newcommand{\ie}{\textit{i.e.}\xspace}
\newcommand{\eg}{\textit{e.g.}\xspace}
\newcommand{\etal}{\textit{et al.}\xspace}
\newcommand{\cf}{\textit{cf.}\xspace}
\newcommand{\vs}{\textit{vs.}\xspace}
\newcommand{\etc}{\textit{etc.}\xspace}
\newcommand{\viz}{\textit{viz.}\xspace}
%\newcommand{\etal}{\textit{et~al.}\xspace}
\newcommand{\lhs}{l.h.s.\xspace}
\newcommand{\rhs}{r.h.s.\xspace}

\newcommand{\mum}{\ensuremath{\mathrm{\mu m}}}
\newcommand{\degree}{\ensuremath{^\circ}\xspace}

%units
\newcommand{\units}[1]{\ensuremath{\,\mathrm{#1}}}


% Convenient ratios and (partial) derivatives
%
%big \frac is called \ratio.
%usage: \ratio{a}{b}
\newcommand{\ratio}[2]{\displaystyle\frac{#1}{#2}}
%usage: \fracd{y}{x} produces fraction dy/dx.
%usage with optional argument: \fracd[2]{y}{x} produces 2nd derivative
\newcommand{\fracd}[3][]{\displaystyle\frac{d^{#1}#2}{d#3^{#1}}}
%usage: \fracp{y}{x} produces partial derivatice dy/dx.
%usage with optional argument: \fracp[2]{y}{x} produces 2nd order partial derivative
\newcommand{\fracp}[3][]{\displaystyle\frac{\partial^{#1}#2}{\partial#3^{#1}}}
%mixed derivatives are not implemented yet :-(

%Averaging macros:
%
%usage1: \av{V} - averaged V
%usage2: \av[x]{V} - V averaged with respect to x
\newcommand{\av}[2][]{\ensuremath{\left\langle#2\right\rangle}_{#1}\xspace}
%usage: \mean{u} - produced bar over the argument
\newcommand{\mean}[1]{\ensuremath{\overline{#1}}\xspace}
\newcommand{\dev}[2][]{\ensuremath{\widetilde{#2}_{#1}}\xspace}

%Freq used materials
\RequirePackage{xspace}
\newcommand{\YBCO}{YBa$_2$Cu$_3$O$_7$\xspace}
\newcommand{\LBCO}[1][x]{La$_{2-#1}$Ba$_#1$CuO$_4$\xspace}
\newcommand{\BSCCO}{Bi$_2$Sr$_2$Ca$_1$Cu$_2$O$_{8}$\xspace}
\newcommand{\NBCO}[1][x]{NdBa$_2$Cu$_3$O$_{7-#1}$\xspace}
\newcommand{\TBCO}{Tl$_2$Ba$_2$CuO$_6$\xspace}
\newcommand{\HBCO}{HgBa$_2$CuO$_6$\xspace}
\newcommand{\NCCO}{Nd$_{2-x}$Ce$_x$CuO$_4$\xspace}
\newcommand{\PCCO}{Pr$_{2-x}$Ce$_x$CuO$_4$\xspace}
\newcommand{\LCMO}[1][x]{La$_{1-#1}$Ca$_x$MnO$_3$\xspace}
\newcommand{\STO}{SrTiO$_3$\xspace}
\newcommand{\CeO}{CeO$_2$\xspace}
\newcommand{\MgB}{MgB$_2$\xspace}
\newcommand{\OrgIJJ}{$\kappa$-(BEDT-TTF)$_2$Cu(NCS)$_2$\xspace}


%technology definitions
\newcommand{\NbAlOxNb}{Nb-AlO$_x$-Nb\xspace}
\newcommand{\TechNb}{Nb-AlO$_x$-Nb\xspace}
\newcommand{\TechYBCONb}{YBCO-Nb\xspace}
%
\newcommand{\SIS}{\ensuremath{\mathrm{S|I|S}}\xspace}
\newcommand{\SNS}{\ensuremath{\mathrm{S|N|S}}\xspace}
\newcommand{\SFS}{\ensuremath{\mathrm{S|F|S}}\xspace}
\newcommand{\SIFS}{S$|$I$|$F$|$S\xspace}
\newcommand{\SfiS}{S$|$FI$|$S\xspace}
%\newcommand{\SJS}{\ensuremath{\mathrm{S-FI-S}}\xspace}

%%
%% Freq used math symbols
%%

%Elliptic fns
\newcommand{\am}{\mathop{\mathrm{am}}\nolimits}
\newcommand{\dn}{\mathop{\mathrm{dn}}\nolimits}
\newcommand{\sn}{\mathop{\mathrm{sn}}\nolimits}
\newcommand{\cn}{\mathop{\mathrm{cn}}\nolimits}
\newcommand{\gd}{\mathop{\mathrm{gd}}\nolimits}
\newcommand{\E} {\mathop{\mathrm{E}}\nolimits}
\newcommand{\F} {\mathop{\mathrm{F}}\nolimits}
\newcommand{\K} {\mathop{\mathrm{K}}\nolimits}
\newcommand{\J}[1][] {\mathop{\mathrm{J_{#1}}}\nolimits}
\newcommand{\Ai} {\mathop{\mathrm{Ai}}\nolimits}
\newcommand{\Bi} {\mathop{\mathrm{Bi}}\nolimits}

%Other fns
%\newcommand{\const}{\mathop{const}\nolimits}
\newcommand{\atanh}{\mathop{\mathrm{atanh}}\nolimits}
\newcommand{\acot}{\mathop{\mathrm{acot}}\nolimits}
\newcommand{\sech}{\mathop{\mathrm{sech}}\nolimits}
\newcommand{\sgn}{\mathop{\mathrm{sgn}}\nolimits}
\newcommand{\floor}{\mathop{\mathrm{floor}}\nolimits}
\newcommand{\const}{\mathop{\mathrm{const}}\nolimits}
\renewcommand{\Re}{\mathop{\mathrm{Re}}\nolimits}
\renewcommand{\Im}{\mathop{\mathrm{Im}}\nolimits}
%\newcommand{\Det}{\mathop{\mathrm{det}}\nolimits}
%\newcommand{\Tr}{\mathop{\mathrm{Tr}}\nolimits}

\newcommand{\qstate}[1]{\ensuremath{\left\lvert\state{#1}\right\rangle}}
\newcommand{\rot}{\mathop\mathrm{\mathbf{rot}}\nolimits}
\newcommand{\grad}{\mathop\mathbf{{\rm grad}}\nolimits}
%\newcommand{\div}{\mathop{{\rm div}}\nolimits}


%just shortcuts
%\newcommand{\HS}{\ensuremath{{\cal H}}}
\newcommand{\Heavyside}{\mathop{\mathrm{H}}\nolimits}
\newcommand{\G}{\ensuremath{{\cal G}}}
\newcommand{\Dx}{\ensuremath{{\Delta x}}}
\newcommand{\dx}{\ensuremath{{\delta x}}}
\newcommand{\Dw}{\ensuremath{{\Delta w}}}
\newcommand{\D}[1]{\ensuremath{{\Delta #1}}}
%\newcommand{\d}[1]{\ensuremath{{\delta #1}}}

%\iffalse%{
\RequirePackage{amssymb}

% macros for showing/hiding corrections

%\RequirePackage[normalem]{ulem}

%\newcommand{\new}[1]{\textcolor{blue}{#1}}
%\newcommand{\del}[1]{\textcolor{red}{\sout{#1}}}
%\newcommand{\chg}[1]{\textcolor{magenta}{#1}}
\RequirePackage{ifthen}
\newboolean{ShowCorrections}
\setboolean{ShowCorrections}{true}%<-- set here show/notshow corrections

%%%Reduction/Corrections macros
\ifthenelse{\boolean{ShowCorrections}}{%
\usepackage[normalem]{ulem}%
\newcommand{\new}[1]{\textcolor[rgb]{0,0,1}{#1}}%
\newcommand{\old}[1]{\textcolor[rgb]{1,0,0}{\sout{#1}}}%
}{%
\newcommand{\new}[1]{#1}%
\newcommand{\old}[1]{}%
}


%%
%% Not allowed stuff
%%

%state command which may not translate correctly
\newcommand{\stat}[1]{\state{#1}}

%%tth:\def\relax{}
%%tth:\def\message#1{}

%\tracingmacros=2
%%%%%%%%%%

\def\state#1{\ensuremath{\stt#1.}}
\def\stt#1{%
\if#1.
\let\next=\relax
\else
  \if#1u
    \upharpoonleft%\uparrow
  \else\if#1d
    \downharpoonleft%\downarrow
  \else\if#1U
    \upharpoonright%\Uparrow
  \else\if#1D
    \downharpoonright%\Downarrow
  \else\if#1F
    \Uparrow
  \else\if#1A
    \Downarrow
  \else\if#1s
    \uparrow
  \else\if#1a
    \downarrow
  \else\if#1r
    \rightarrow
  \else\if#1l
    \leftarrow
  \else\if#1R
    \Rightarrow
  \else\if#1L
    \Leftarrow
  \else\if#1>
    \longrightarrow
  \else\if#1<
    \longleftarrow
  \else\if#1
  \relax
  \else
  ?\message{Unknown symbol #1 in the argument of macro state}
  \fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi
\let\next=\stt
\fi
\next
}

%usage: \hstruct{Nb|Al|Nb}
%at the moment cannot accept math or lower indices. :-(
\def\hstruct#1{%
\let\accu=\relax%
\hstruc#1.%
\accu
}
\def\hstruc#1{%
\if#1.%end?
\let\next=\relax
\else
  \if#1|%
    \let\accu=\accu$|$%
%  \else\if#1
%    \relax
  \else
    \let\accu=\accu #1%\message{Unknown symbol #1 in the argument of macro \hstruc}
  \fi%\fi
  \let\next=\hstruc
\fi
\next
}


\newcounter{CurrTimeHH}\newcounter{CurrTimeMM}
\newcommand{\CurrTime}{%
  \setcounter{CurrTimeHH}{\time/60}%
  \setcounter{CurrTimeMM}{\time - \value{CurrTimeHH}*60}%
  \ifthenelse{\value{CurrTimeHH}<10}{0}{}\theCurrTimeHH:%
  \ifthenelse{\value{CurrTimeMM}<10}{0}{}\theCurrTimeMM%
}




==> we.tex <==
%Misc. macros to discuss with co-authors
\RequirePackage{color}
\newcommand{\HS}[1]{{\textcolor{red}{\textbf{HS:``#1''}}}}
\newcommand{\EG}[1]{{\textcolor[rgb]{1,.4,0}{\textbf{EG:``#1''}}}}
\newcommand{\DK}[1]{{\textcolor[rgb]{0,0.7,0}{\textbf{DK:``#1''}}}}
\newcommand{\RK}[1]{{\textcolor[rgb]{1.0,0,0}{\textbf{RK:``#1''}}}}
\newcommand{\RM}[1]{{\textcolor[rgb]{0.4,.4,1}{\textbf{RM:``#1''}}}}

